Deep Analysis of CNN-based Spatio-temporal Representations for Action Recognition

In recent years, a number of approaches based on 2D or 3D convolutional neural networks (CNN) have emerged for video action recognition, achieving state-of-the-art results on several large-scale benchmark datasets. In this paper, we carry out in-depth comparative analysis to better understand the differences between these approaches and the progress made by them. To this end, we develop an unified framework for both 2D-CNN and 3D-CNN action models, which enables us to remove bells and whistles and provides a common ground for fair comparison. We then conduct an effort towards a large-scale analysis involving over 300 action recognition models. Our comprehensive analysis reveals that a) a significant leap is made in efficiency for action recognition, but not in accuracy; b) 2D-CNN and 3D-CNN models behave similarly in terms of spatio-temporal representation abilities and transferability. Our codes are available at https://github.com/IBM/action-recognition-pytorch.

==> Main/tables/cls_acc_correlation.tex <==
\begin{table}[t]
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{c|c|c|}
        \toprule
             TAM <--> I3D  &  TAM <--> Slowfast  &  I3D <--> Slowfast \\ 
        \midrule
             0.8419& 0.7861  & 0.7772 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    % \vspace{-2mm}
    \caption{Class accuracy correlations.}
    \label{table:class_acc_correlations}
\end{table}

==> Main/tables/comparison_table.tex <==

\begin{table}[tb]
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{l|c|c|c|c}
\toprule
                                                       Approaches &      Backbone &        Frames &    Resolution &    Evaluation \\
\midrule
                                  C3D~\cite{C3D:Tran2015learning} &  $\checkmark$ &  $\checkmark$ &               &               \\
                                  TSN~\cite{TSN:wang2016temporal} &               &               &               &               \\
                                   I3D~\cite{I3D:carreira2017quo} &  $\checkmark$ &  $\checkmark$ &               &               \\
                                     P3D~\cite{P3D:Qiu_2017_ICCV} &  $\checkmark$ &  $\checkmark$ &               &               \\
                                    STC~\cite{STC:Diba2018spatio} &  $\checkmark$ &  $\checkmark$ &  $\checkmark$ &               \\
                              Res3D~\cite{ResNet3D_2:hara2018can} &  $\checkmark$ &  $\checkmark$ &  $\checkmark$ &               \\
                          ARTNet~\cite{ARTNet:Wang2018appearance} &  $\checkmark$ &  $\checkmark$ &  $\checkmark$ &               \\
                                 ECO~\cite{ECO:zolfaghari2018eco} &  $\checkmark$ &  $\checkmark$ &               &  $\checkmark$ \\
                        NonLocal~\cite{Nonlocal:Wang2018NonLocal} &  $\checkmark$ &  $\checkmark$ &               &  $\checkmark$ \\
                           R(2+1)D~\cite{R2plus1D:Tran_2018_CVPR} &  $\checkmark$ &               &  $\checkmark$ &               \\
                                                   S3D~\cite{S3D} &               &               &               &               \\
                                    CSN~\cite{CSN:Tran_2019_ICCV} &  $\checkmark$ &  $\checkmark$ &               &               \\
                 Timeception~\cite{Timeception:Hussein_CVPR_2019} &  $\checkmark$ &  $\checkmark$ &               &               \\
                                   STNet~\cite{StNet:He:2019aaai} &  $\checkmark$ &               &               &               \\
                                             TAM~\cite{bLVNetTAM} &  $\checkmark$ &               &               &  $\checkmark$ \\
                                   TSM~\cite{TSM:lin2018temporal} &  $\checkmark$ &  $\checkmark$ &               &  $\checkmark$ \\
                          CST~\cite{CollaborativeST:Li_2019_CVPR} &  $\checkmark$ &  $\checkmark$ &               &               \\
                                     GST~\cite{GST:Luo_2019_ICCV} &               &               &               &               \\
               SlowFast~\cite{SlowFast:feichtenhofer2018slowfast} &               &  $\checkmark$ &               &               \\
                            CorrNet~\cite{CorrNet:Wang_2020_CVPR} &               &  $\checkmark$ &               &               \\
 TEINet~\cite{TEINet:Liu_Luo_Wang_Wang_Tai_Wang_Li_Huang_Lu_2020} &  $\checkmark$ &               &               &  $\checkmark$ \\
                     RubiksNet~\cite{RubiksNet:fanbuch2020rubiks} &               &               &               &               \\
                           X3D~\cite{X3D_Feichtenhofer_2020_CVPR} &  $\checkmark$ &  $\checkmark$ &  $\checkmark$ &               \\
\bottomrule
\end{tabular}
    \end{adjustbox}
    % \vspace{-2mm}
    \caption{A summary of the comparison made by the recent papers for action recognition. $\checkmark$ denotes there are differences when the paper compares to others. E.g., the backbone column means that the papers compare the results with different backbones. Hence, many papers are compared with mixed backbones, distinct frame numbers, or evaluation differently.}
    \label{table:compare}
\end{table}


==> Main/tables/full_dataset.tex <==

\begin{table}
    % \vspace{-10pt}
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{c|c|c|c|cc|c|c|c|cc|cc|cc|cc}
        \toprule
        \multirow{2}{*}{Approach} & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Sampling} & \multirow{2}{*}{TP}& \multicolumn{2}{c|}{Frame \#} &\multirow{2}{*}{Pretrained} & \multirow{2}{*}{Params} & \multirow{2}{*}{FLOPs$^\dagger$} & \multicolumn{2}{c|}{SSV2 (\textbf{clip})} & \multicolumn{2}{c}{SSV2 (\textbf{video})} & \multicolumn{2}{c|}{Kinetics (\textbf{clip})} & \multicolumn{2}{c}{Kinetics (\textbf{video})} \\
        \cmidrule{5-6} \cmidrule{10-17}
        &   & & & Train & Eval.  & & & &  Top-1   & Top-5     &   Top-1   &   Top-5  &  Top-1   & Top-5     &   Top-1   &   Top-5\\
        \midrule
        \multirow{4}{*}{I3D} & \multirow{2}{*}{InceptionV1} & \multirow{4}{*}{uniform} & \multirow{4}{*}{Y} & 16 &16$\times$10 &imagenet & \multirow{2}{*}{12.5M} & 42.8G &50.0 & 78.8 & 51.1 & 79.9 & 63.3 & 84.8 & 64.2 & 85.7 \\
            & & & & 64  &64$\times$10 & imagenet&  & 171.2G & 62.3 & 88.8 & 62.7 & 89.1 &  68.0 & 88.5 & 68.1 & 88.6\\
            \cmidrule{2-2}\cmidrule{5-17}
            & \multirow{2}{*}{ResNet50} & & & 16 &16$\times$10 &imagenet & \multirow{2}{*}{46.6M}  & 58.9G & 52.6 & 80.4 & 53.6 & 81.6 & 67.1 & 86.9 & 68.1 & 87.9\\
            & & & & 64 & 64$\times$10 &imagenet  & & 235.6G & 64.1 & 89.8 & 64.7 & 90.2 & 72.1 & 90.5 & 72.3 & 90.6\\
        \midrule
        \multirow{4}{*}{S3D} & \multirow{2}{*}{InceptionV1}& \multirow{4}{*}{uniform} & \multirow{4}{*}{Y} & 16 &16$\times$10 &imagenet & \multirow{2}{*}{8.1M} & 24.5G &52.7 & 81.4 & 53.8 & 82.4 &  62.8 & 85.0 & 63.9 & 85.8\\
            & & & & 64 & 64$\times$10& imagenet  & & 98.1G & 61.9 & 88.8 & 62.5 & 89.3 & 68.2 & 88.6  & 68.5 & 88.9\\
            \cmidrule{2-2}\cmidrule{5-17}
            & \multirow{2}{*}{ResNet50} & &  & 16 &16$\times$10  &imagenet & \multirow{2}{*}{27.7M} & 39.3G & 52.2 & 80.3 & 53.4 & 81.5 &  65.8 & 86.4 & 66.8 & 87.3\\
            & & & &  64 &64$\times$10  &imagenet  & & 157.3G & 63.6 & 89.6 & 64.2 & 90.0 & 70.9 & 89.9 & 71.2 & 90.1\\
        \midrule
        \multirow{4}{*}{TSN} & \multirow{2}{*}{InceptionV1} & \multirow{4}{*}{uniform} &\multirow{4}{*}{N} & 16 &16$\times$10 &imagenet  & \multirow{2}{*}{5.8M} & 24.0G & 30.6 & 62.1 & 31.1 & 62.4 & 65.2 & 86.4 & 65.6 & 86.4 \\
            & & &  & 64 &64$\times$10 & imagenet  & & 95.8G & 24.7 & 53.8 & 24.6 & 54.1 & 64.3 & 85.5 & 64.2 & 85.5\\
            \cmidrule{2-2}\cmidrule{5-17}
            & \multirow{2}{*}{ResNet50} & &  & 16 & 16$\times$10& imagenet & \multirow{2}{*}{23.9M} & 65.4G & 30.7 & 61.6 & 30.8 & 62.0 & 67.3 & 87.6 & 67.7 & 87.9 \\
            & & & & 64 &64$\times$10  & imagenet & & 261.6G & 29.4 & 60.6 & 29.6 & 61.0 & 67.9 & 88.1 & 68.0 & 88.1 \\
        \midrule        
        \multirow{4}{*}{TAM} & \multirow{2}{*}{InceptionV1} &\multirow{4}{*}{uniform} & \multirow{4}{*}{N} &16 & 16$\times$10 & imagenet& \multirow{2}{*}{5.8M} & 24.1G &58.6 & 86.1 & 59.3 & 86.8 & 66.7 & 87.6 & 67.3 & 88.1 \\
            & & & &  64 & 64$\times$10  &imagenet &   & 96.3G &60.3 & 87.7 & 61.0 & 88.0 & 68.5 & 88.8 & 68.6 & 88.9\\
            \cmidrule{2-2}\cmidrule{5-17}
            & \multirow{2}{*}{ResNet50} & & & 16 &16$\times$10&imagenet& \multirow{2}{*}{24.0M} & 65.7G & 61.9 & 88.2 & 62.8 & 88.5 & 68.4 & 88.2 & 69.0 & 88.7 \\
            & & & & 64 &64$\times$10 &imagenet & & 262.7G &64.6 & 90.3 & \textbf{65.1} & \textbf{90.5} & 73.9 & 91.6 & \textbf{74.1} & \textbf{91.6} \\
        \midrule
        \midrule       
        \multirow{2}{*}{I3D*} & InceptionV1~\cite{I3D:carreira2017quo} &\multirow{2}{*}{dense} & \multirow{2}{*}{Y} & 64 &250 &imagenet & 12.1M & 107.9G & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ &71.1 & 89.3\\
            &ResNet50~\cite{ResNet3D_2:hara2018can} & & & 16 &N/A &none& $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ &61.3 &83.1\\
        \midrule       
        \multirow{4}{*}{S3D*} & InceptionV1~\cite{S3D} &\multirow{3}{*}{dense} & \multirow{3}{*}{Y} & 64 &250 &imagenet& 8.8M & 66.4G  & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ &72.2 & 90.6\\
            &ResNet34~\cite{R2plus1D:Tran_2018_CVPR} & & & 16 &16$\times$10 &none & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ &72.2&90.6 \\
            &ResNet34~\cite{R2plus1D:Tran_2018_CVPR} & & & 16 &16$\times$10 &sports1M & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ &74.7&93.4 \\
        \midrule       
    %    \multirow{2}{*}{TSN*} & InceptionV1~\cite{TSN:wang2016temporal} & \multirow{2}{*}{Y} & N/A && imagenet &  & & & & & &  &  &69.1 &88.7 \\
    %        &InceptionV1~\cite{TSN:wang2016temporal} & & N/A & &imagenet & & & &  & & &   &  & 72.5&90.2\\
    %    \midrule       
        TAM* &bLResNet50~\cite{bLVNetTAM} & uniform & N & 32 &32 & imagenet& \multirow{2}{*}{25.0M} & 47.7G & 61.7 & 88.1 & $-$ & $-$ & $-$ & $-$ & $-$ & $-$\\
        TAM* &bLResNet50~\cite{bLVNetTAM} & uniform & N & 48 &48$\times$9& imagenet&  &  93.4G & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ &73.5&91.2\\
        \bottomrule
        \multicolumn{17}{l}{\footnotesize{$\dagger$: The FLOPs is conducted based on number of frames used in training. *: results from the original papers.}} \\
    \end{tabular}
    \end{adjustbox}
    % \vspace{-2mm}
    \caption{Clip- and video-level accuracies of different models on SSV2 and Kinetics400}
    \label{table:acc_full_set}
\end{table}


==> Main/tables/i3d-r50s.tex <==

\begin{table}[tb]
\begin{adjustbox}{max width=\linewidth}
\centering
    \begin{tabular}{cc|cccc}
    \toprule
    Dataset & InceptionV1-tp & R50-tp & R50 & SE-R50 & SlowFast-R50/TAM-R50 \\
    \midrule
    \Kinetics & 71.40 & 75.49 (+4.09) & 76.61 (+1.12) & \textbf{77.79 (+1.18)} & 77.0 \\
    \SSV2 & 56.81 & 56.82 (+0.01) & 62.84 (+6.02) & 62.71 (-0.13) & 63.83 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    % \vspace{-2mm}
    \caption{Performance (Top-1 Acc. (\%)) of I3D models with different settings on \Kinetics (backbone, temporal pooling and squeeze-excitation layer). All models are trained under 32 frames and the same training protocol.}
    \label{table:i3d-r50s}
\end{table}


==> Main/tables/input_sampling.tex <==
\begin{table}[bt]
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{c|c|c|cc|cc}
        \toprule
        Dataset & Approach & Backbone & \multicolumn{2}{c|}{Dense (\textbf{video-level})} & \multicolumn{2}{c}{Uniform (\textbf{video-level})} \\
        \cmidrule{4-7}
      & & &Top-1   & Top-5   &   Top-1   &   Top-5\\
        \midrule
    % \multicolumn{6}{c}{Mini Kinetics400} \\
    % \midrule
    \multirow{4}{*}{\mKinetics}& I3D &ResNet18 & 69.3 & 88.3 & 68.0 & 87.6\\
    % I3D &IncpetionV1 & 58.9 & 79.7 & 71.8 & 89.6 & 68.1 & 87.6 & & \\
    & &IncpetionV1 & 70.8 & 89.6 &  69.1 & 88.3 \\
    \cmidrule{2-7}
    & TAM &ResNet18    & 67.7 & 87.5 &  69.8 & 88.9\\
    % TAM &ResNet50    & 62.4 & 82.1 & 75.0 & 91.2 & 74.1 & 90.4 & 75.2 & 91.0\\
    & &ResNet50    & 74.2 & 91.0 & 75.2 & 91.0\\
    
    % \midrule
    % \midrule
    % \multicolumn{6}{c}{Mini SSV2} \\
    \midrule
    \multirow{4}{*}{\mSSV2} & I3D &ResNet18    & 42.1 & 72.1 & 57.1 & 82.8\\
    & &IncpetionV1 & 46.1 & 75.4 & 58.0 & 83.8 \\
    \cmidrule{2-7}
    & TAM &ResNet18    & 47.2 & 77.1 & 60.6 & 86.2 \\
    & &ResNet50    & 52.4 & 80.9 & 67.2 & 89.8 \\
    \bottomrule
        % \multicolumn{8}{l}{\footnotesize{There is a performance of I3D and S3D from the original paper is b}}
    \end{tabular}
    \end{adjustbox}
    % \vspace{-2mm}
    \caption{\small {Video-level accuracies on \mKinetics and \mSSV2.} }
    \label{table:input_sampling}
\end{table}

==> Main/tables/sota_moments.tex <==
\begin{table}[tb]
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{c|c|c}
        \toprule
            Model & Pretrain & Top-1 Acc.\\
            \midrule
            I3D-ResNet50 & ImageNet & 31.21 \\ % 256.7G
            TAM-ResNet50 & ImageNet & 30.80 \\ % 131.3G
            SlowFast-ResNet50-8$\times$8$^\dagger$ & $-$ & 31.20  \\
            \midrule
            MiT~\cite{Moments:monfort2019moments}$^{*}$ & ImageNet & 31.16 \\
            AssembleNet-50$\ddagger$~\cite{AssembleNet:Ryoo2020AssembleNet_ICLR2020} & $-$ & 31.41 \\
            GST-ResNet101~\cite{CollaborativeST:Li_2019_CVPR} & ImageNet & 32.40 \\
        \bottomrule
        \multicolumn{3}{l}{\footnotesize{$^\dagger$: Trained by ourselves. $^\ddagger$: use both RGB and Flow.} } \\
        \multicolumn{3}{l}{\footnotesize{$^{*}$: Use RGB+Flow+Audio and mixed networks} } \\
    \end{tabular}  
    \end{adjustbox}
    % \vspace{-2mm}
    \caption{Performance of SOTA models on \Moments. All models use 32 frames except MiT.}
    \label{table:sota_mit}
\end{table}

==> Main/tables/spatio_temporal_modeling_backbone.tex <==

\begin{table}[t]
    % \vspace{-10pt}
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
        \toprule
        \multirow{2}{*}{Datasets} & \multirow{2}{*}{Metrics} & \multicolumn{3}{c|}{S3D} & \multicolumn{3}{c|}{I3D} & \multicolumn{3}{c}{TAM}  \\
        \cmidrule{3-11}
                 &         & InceptionV1 & ResNet18 & ResNet50  & InceptionV1 & ResNet18 & ResNet50 & InceptionV1 & ResNet18 & ResNet50  \\
        % \cmidrule{2-7}
        \midrule
        Mini-       &   $\Phi_a^b$        &  0.55 & 0.49 & 0.54 & 0.56 & 0.51 & 0.54 & 0.54 & 0.50 & 0.52 \\
        SSV2        &   $\Psi_a^{b^{ta}}$ &  0.44 & 0.47 & 0.47 & 0.43 & 0.44 & 0.48 & 0.45 & 0.45 & 0.52 \\
        \midrule
        Mini-       &   $\Phi_a^b$        &  0.98 & 0.96 & 0.97 & 0.97 & 0.96 & 0.96 & 0.98 & 0.96 & 0.95 \\
        Kinetics    &   $\Psi_a^{b^{ta}}$ &  0.02 & 0.09 & 0.07 & 0.05 & 0.07 & 0.11 & 0.04 & 0.09 & 0.14 \\
        \midrule
        Mini-       &   $\Phi_a^b$        &  0.93 & 0.85 & 0.88 & 0.91 & 0.94 & 0.89 & 0.89 & 0.88 & 0.84\\
        Moments     &   $\Psi_a^{b^{ta}}$ &  0.02 & 0.05 & 0.04 & 0.03 & 0.02 & 0.04 & 0.04 & 0.04 & 0.06\\
        \bottomrule
        % \multicolumn{8}{l}{\footnotesize{$\bar{\Psi}_a^{b^{tp}}$: effects from temporal pooling.}} \\
        \multicolumn{8}{l}{\footnotesize{$\Psi_a^{b^{ta}}$: the improvement from temporal aggregation.}}
    \end{tabular}
    \end{adjustbox}
    % \vspace{-2mm}
    \caption{\small Spatiotemporal modeling by different backbones w/o temporal pooling.}
    \label{table:spt_modeling_backbone}
    
\end{table}


==> Main/tex/training_details.tex <==
\section{Implementation Details}
\label{sec:suppl:protocol}



% \subsection {Implementation} \label{sec:impl}
We follow the original published papers as much as we can to implement the approaches in our analysis. However, due to the differences in backbones, some modifications are necessary to ensure a fair comparison under a common experimental framework. 
Here we describe how we build the networks including three backbones (InceptionV1, ResNet18 and ResNet50), four video architectures (I3D, S3D, TAM and TSN), and where to perform temporal pooling.
% First, we explain the general concept for each one and then details the difference from the original paper.
For three backbones, we used those 2D models available on the torchvision repository (\textit{googlenet, resnet18, resnet50}), and then used the weights in the model zoo for initializing models either through inflation (I3D and S3D) or directly loading (TAM and TSN). Note that, for inflation, we simply copy the weights along the time dimension.
%For temporal pooling, to perform fair comparison, 
Moreover, we always perform the same number of temporal poolings at the similar locations across all backbones for temporal pooling. For each backbone, there are five positions to perform \textit{spatial pooling}, we add maximum \textit{temporal pooling} along with the last three spatial poolings (kernel size is set to 3).

% \vspace{1mm}
\noindent
\textbf{I3D.} We follow the original I3D paper to re-implement the network~\cite{I3D:carreira2017quo}. We convert all 2D convolutional layer into 3D convolutions and set the kernel size in temporal domain to 3 while using the same spatial kernel size. For I3D-ResNet-50, we convert the 3$\times$3 convolution in the bottleneck block into 3$\times$3$\times$3.

% \vspace{1mm}
\noindent
\textbf{S3D.} We follow the idea of the original S3D and R(2+1)D paper to factorize 3D convolution in the re-implemented models~\cite{S3D,R2plus1D:Tran_2018_CVPR}; thus, each 3D convolution in I3D becomes one 2D spatial convolution and one 1D temporal convolution. Nonetheless, the first convolution of the network is not factorized as the original papers. For InceptionV1 backbone, the difference from the original paper is the location of temporal pooling of backbone~\cite{S3D}. More specifically, in our implementation, we remove the temporal stride in the first convolutional layer and then add an temporal pooling layer to keep the same temporal downsampling ratio over the model. On the other hand, for ResNet backbone, 
we do not follow the R(2+1)D paper to expand the channels to have similar parameters to the corresponding I3D models, 
we simply set the output channels to the original output channel size~\cite{R2plus1D:Tran_2018_CVPR} which helps us to directly load the ImageNet-pretrained weights into the model.

% \vspace{1mm}
\noindent
\textbf{TAM.} We follow the original paper to build TAM-ResNet~\cite{bLVNetTAM}, the TAM module is inserted at the non-identity path of every residual block. On the other hand, for TAM-InceptionV1, we add TAM modules after the every inception module.

\begin{figure*}[tb!]
    \centering
    \includegraphics[width=\linewidth]{images/all_results_wtp.pdf}
    \caption{Top-1 accuracy of all models with and without temporal pooling on three mini-datasets. The video architectures are separated by color while the backbones by symbol. Best viewed in color.}
    \label{fig:all_results_wtp}
\end{figure*}


\vspace{1mm}
\noindent
\textbf{TSN.} It does not have any temporal modeling, so it directly uses 2D models.


